Strategic Reasoning with Language Models

Strategic reasoning enables agents to cooperate, communicate, and compete with other agents in diverse situations. Existing approaches to solving strategic games rely on extensive training, yielding strategies that do not generalize to new scenarios or games without retraining. Large Language Models (LLMs), with their ability to comprehend and generate complex, context-rich language, could prove powerful as tools for strategic gameplay. This paper introduces an approach that uses pretrained LLMs with few-shot chain-of-thought examples to enable strategic reasoning for AI agents. Our approach uses systematically generated demonstrations of reasoning about states, values, and beliefs to prompt the model. Using extensive variations of simple matrix games, we show that strategies that are derived based on systematically generated prompts generalize almost perfectly to new game structures, alternate objectives, and hidden information. Additionally, we demonstrate our approach can lead to human-like negotiation strategies in realistic scenarios without any extra training or fine-tuning. Our results highlight the ability of LLMs, guided by systematic reasoning demonstrations, to adapt and excel in diverse strategic scenarios.

==> prompts/broker.tex <==
\begin{figure*}[hbtp]

\vspace{-1cm}
    \caption{A demonstration of a broker trying to find a Rawlsian fair dail with iterated action selection.}
    \label{prompt:neg}
\begin{tcolorbox}[
    prompt,
    title={\small \textbf{A demonstration of a broker trying to find a Rawlsian fair dail with iterated action selection.}},
    width=\textwidth]
    \fontsize{7pt}{7pt}\selectfont
## New Deal
items available:
book=3
hat=1
ball=2
Bob's values: book: 0, hat: 2, ball: 4
Alice's values: book: 1, hat: 3, ball: 2
Q: What is a proposal that is Rawlsian fair? Try at most 3 proposals.
Try 1/3.
items: book=3, hat=1, ball=2
Bob values: ball:4 > hat:2 > book:0
Alice values: hat:3 > ball:2 > book:1
For a Rawlsian fair proposal, Alice gets 3/3 books, 1/1 hats, 0/2 balls.
So, Bob gets (3-3)=0 books, (1-1)=0 hats, (2-0)=2 balls.
Value of proposal for Alice:  (3*1) + (1*3) + (0*2) = 3+3+0 = 6/10
Value of proposal for Bob:  (0*0) + (0*2) + (2*4) = 0+0+8 = 8/10
Alice gets 6/10 and Bob gets 8/10. The lower payoff 6/10 can be improved.
So, let's try again.
Try 2/3.
items: book=3, hat=1, ball=2
Bob values: ball:4 > hat:2 > book:0
Alice values: hat:3 > ball:2 > book:1
For a Rawlsian fair proposal, Alice gets 2/3 books, 1/1 hats, 1/2 balls.
So, Bob gets (3-2)=1 books, (1-1)=0 hats, (2-1)=1 balls.
Value of proposal for Alice:  (2*1) + (1*3) + (1*2) = 2+3+2 = 7/10
Value of proposal for Bob:  (1*0) + (0*2) + (1*4) = 0+0+4 = 4/10
Alice gets 7/10 and Bob gets 4/10. The lower payoff 4/10 is too low.
So, let's try again.
Try 3/3.
items: book=3, hat=1, ball=2
Bob values: ball:4 > hat:2 > book:0
Alice values: hat:3 > ball:2 > book:1
For a Rawlsian fair proposal, Alice gets 1/3 books, 1/1 hats, 2/2 balls.
So, Bob gets (3-1)=2 books, (1-1)=0 hats, (2-2)=0 balls.
Value of proposal for Alice:  (1*1) + (1*3) + (2*2) = 1+3+4 = 8/10
Value of proposal for Bob:  (2*0) + (0*2) + (0*4) = 0+0+0 = 0/10
Alice gets 8/10 and Bob gets 0/10. The lower payoff 0/10 is too low.
Summary of tries:
Try 1/3: Alice gets 6/10 and Bob gets 8/10. The lower payoff 6/10.
Try 2/3: Alice gets 7/10 and Bob gets 4/10. The lower payoff 4/10.
Try 3/3: Alice gets 8/10 and Bob gets 0/10. The lower payoff 0/10.
Highest lower payoff of max(6, 4, 0) = 6. So, we go with try 1/3. Alice gets 3 books, 1 hats, 0 balls.
propose: book=3 hat=1 ball=0
\normalfont
\end{tcolorbox}
\end{figure*}

==> sections/11_checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?\answerYes{}
  \item Did you describe the limitations of your work? \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work? \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results? \answerNA{}
        \item Did you include complete proofs of all theoretical results? \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators? \answerYes{}
  \item Did you mention the license of the assets? \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL? \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating? \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?  \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \answerYes{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \answerYes{}
\end{enumerate}


\end{enumerate}

==> sections/backups/04a_back.tex <==
In this section, we show how language models guided with demonstrations generated from our method can learn to solve novel game trees reliably, generalizing to new rules and structures. 
\vspace{-0.2cm}
\subsubsection{Matrix Games: New Rewards, Structures} \label{subsec:sim}
Here, we focus on testing generalization to new game structures and rewards; games with more players, more actions and new reward functions. The objective of the players is to maximize their rewards. The players play their actions simultaneously. We assume that the model is playing against a na\"ive (level-0) player (this is specified in the instruction). 

\textbf{In-Context Demonstrations.}  We use two trivial $2\times 2$ matrix games to teach the model how to search and reason. One of these matrix games has payoffs that are purely in a descending order ($8,7\dots1$). The other game has payoffs that teach the model how to reason in the case of a tie; when two actions have the same reward.

\textbf{Evaluation Tasks.} To evaluate generalization to new rewards, we evaluate the model on 7 types of matrix games: Prisoner's dilemma, chicken, stag hunt, battle of the sexes, a market entry game, imbalanced matching pennies, and deadlock (see \autoref{asec:22mat}). These games are chosen since they require different types of behaviors to be successful; like cooperation, compromise, and adversarial action. We use 5 variations of payoffs for each of these games to get a total of 35 games. 

\kg{move to section on fatoring?}Next, to test generalization to new game structures, the model is evaluated on 15 games of three different structures, with more actions $3\times 3$, with asymmetric actions $4\times 3$, with more players $2\times 2\times 2$. The payoffs for these games are extended versions of their $2\times2$ versions (sup. \autoref{afig:matrix-more}). For example, we use a 3-way prisoner's dilemma and chicken game to evaluate generalization to games with more players.

\textbf{Results.} Language models prompted to systematically search and assign values with our method generalize successfully to new payoffs (see \autoref{tab:search}). Based on the payoffs, models are able to express different types of behaviors. Vanilla strategies of prompting such as 0-shot, 2-shot, and 0-shot CoT prompts are less successful at generalizing to new payoffs. Further, when we ablate the strategic prompt to  remove parts of search or value assignment, performance becomes less reliable; showing how parts of our reasoning structure help in making LLMs more reliable. This result also holds for games where actions are taken sequentially (see \autoref{subsec:seq}). Further, we see that reasoning from in-context demonstrations allows models to flexibly generalize to game with more players and actions without any demonstrations for the new game structures, achieving an almost perfect score 0.96 (43/45). Failures of our approach usually involve errors in comparing rewards such as: ``-1.0 > 0.0''.
\vspace{-0.15cm}
\subsubsection{Combination of sequential and simultaneous games}
\label{subsec:complex}
In this section, we show how our method can be used to teach new games to LLMs with a small number of demonstrations. To test this, we consider games with multiple rounds and varying formats of play. In the first game structure, players play a simultaneous action game and then a sequential action game (see \autoref{asec:complex}). Analogously, in another evaluation, the players first play a simultaneous game and then a sequential one. Similar to previous sections, the opponent is assumed to be a na\"ive player. 

\textbf{In-Context Demonstrations.} We provide two in-context demonstrations for the new game structure with trivial payoffs to show how to reason with a new structure.

\textbf{Evaluation Tasks.} We test the model on two forms of payoffs with 5 variations each (see \autoref{asec:complex}). We do this for both the simultaneous-sequential and the sequential-simultaneous game trees.

\textbf{Results.} The model successfully (\autoref{tab:search}) generalizes to new payoffs with one in-context demonstration of reasoning over the novel game tree. Our demonstration of how our method enables LLMs to quickly generalize
to new tasks suggests that it may be useful in other domains where the ability to quickly adapt to new information is valuable.

\subsubsection{Factoring Strategic Reasoning}
\label{subsec:factor}
\kg{add description}
 \begin{table}[!hbt]
     \centering
     \begin{tabular}{lc}
     \toprule
        Method  &  \\
        \midrule
         No Factor &  \\
         Factor &  \\
         \bottomrule
     \end{tabular}
     \caption{Comparison of accuracies of predicting the best response with and without factored reasoning.\kg{update table/figure}}
     \label{tab:factor}
 \end{table}


\begin{table}[tpb]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccc}
    \toprule
       Objectives  & 0-shot & 0-shot CoT  & 2-shot & Strategic & No Search & No Value\\
       \midrule
        Max, Max & 0.29 (10/35)& 0.49 (17/35) &0.37 (13/35) & \textbf{1.0} (35/35)& 0.66 (23/35)& 0.88 (31/35)\\
        Max, Help  & 0.51 (18/35) &0.63 (22/35) & 0.49 (17/35)& \textbf{1.0} (35/35) &0.69 (24/35)&0.77 (27/35)\\
        Help, Max & 0.03 (1/35) & 0.51 (18/35)  & 0.43 (15/35) & \textbf{1.0} (35/35)&0.20 (7/35)& 0.63 (22/35)\\
        Welfare, Welfare & 0.63 (22/35) & 0.66 (23/35) &  0.60 (21/35) & \textbf{1.0} (35/35)&0.51 (18/35)&0.63 (22/35)\\
        Daxity, Daxity & 0.23 (8/35)& 0.43 (15/35)& 0.43 (15/35) & \textbf{0.94} (33/35)&0.60 (21/35) &0.71 (25/35)\\
    \bottomrule 
    \end{tabular}
    \end{adjustbox}
    \caption{Accuracy of choosing the best response for a new objective that has never been seen before. The goals in the first column indicate the objectives of the model and its opponent respectively; ``max, help'' means that the model is trying to maximize its payoff while its opponent is trying to help the model maximize the payoff. Daxity indicates a new objective that we define to be the difference between the payoff received by the player and its opponent.}
    \label{tab:value}
\end{table}

\textbf{In-Context Demonstrations.} 

\textbf{Evaluation Tasks.} 

\textbf{Results.} \kg{reference k-level reasoning here.}

==> sections/backups/04c_back.tex <==
\begin{figure*}
    \centering
\includegraphics[width=\textwidth]{figures/neg-prompts-strat.pdf}
    \caption{A sample episode (a) from Deal or No Deal \citep{lewis2017deal} with a (b) demonstration of the reasoning prompt; red indicates reasoning over values, green indicates search, and yellow indicates beliefs.}
    \label{fig:dealnodeal}
\end{figure*}
In this section, we show  how LLMs prompted with our method to track beliefs can solve games with a variety of partially observable information, like hidden states, veracity of communication and understanding an opponent's values.

\vspace{-0.1cm}
\subsubsection{Beliefs over States}
In this section we introduce partial observability in the state of the world. We consider a sequential game where the player (model) cannot see the state of the world but can see the action that their opponent takes, and the payoffs that they receive for different world states. So, the player can observe the opponent's actions and values and must form a belief over the world state from these. We consider three types of game trees; (see \autoref{fig:front}) to show how language can be used for forming beliefs about hidden information. We show the prompt structure in \autoref{fig:front}. We evaluate their performance based on choosing the best response (response with the highest payoff).

\textbf{In-Context Demonstrations.} To demonstrate reasoning over hidden states of the world, we use 2 examples of games with trivial payoffs (similar to previous sections). 

\textbf{Evaluation Tasks.} We use three game structures with five variations of payoffs to test generalization. The first game structure is the same as the in-context demonstrations but with non-trivial payoffs. In the second structure, the world has three hidden states instead of two. For the final structure, the number of actions that the opponent can take is increased from two to three.

\textbf{Results.} Models with our structures of reasoning outperform other baselines, generalizing to new structures with no demonstrations. Here, we show how in-context demonstrations can guide language models to update beliefs about the world based on evidence.

\begin{figure*}[!hbtp]
    \centering
\includegraphics[width=\textwidth]{figures/neg-plots-strat.pdf}
    \caption{Comparison of different methods on different metrics when paired with real humans in the Deal or No Deal task. We show how our method outperforms baselines and ablations in human user studies. Error bars represent the standard deviation.}
    \label{fig:deal-res}
\end{figure*}
\subsubsection{Beliefs of Truthfulness}
\kg{move to appendix}
Here, we consider games where the opponent can communicate with the player and tell them what action they are going to play. The opponent can be faithful to what they say they are going to play or lie about their intentions. The player must infer if their opponent is telling the truth or is lying based on the payoffs, and then choose the best response to their opponents actions. We show how language can help understand and reason over the veracity of communication. Veracity can be seen as a hidden state of the world (the opponent) that the model must infer from the evidence. We use a reasoning structure similar to the previous section. The opponent in our evaluations is na\"ive, and assumes that the player will believe whatever they are told.

\textbf{In-Context Demonstrations.} We use one demonstration with trivial payoffs to teach the model to form a belief over the honesty of the communication. In this demonstration, the opponent says the truth. We use a second demonstration with trivial payoffs to teach the model how to break ties (same as \autoref{subsec:sim}).

\textbf{Evaluation Tasks.} We test the model on 5 types of $2\times 2$ matrix games (cooperation, matching pennies, prisoner's dilemma, chicken, battle of the sexes; see \autoref{asec:matrix}) with 5 variations of payoffs. These games are designed such that some require deception while others rely on the honesty of communication.

\textbf{Results.} We find that models that search through different states of the world based on the payoffs and actions are able to infer the veracity of the communication reliably. The model is successful in generalizing to new payoff structures and to scenarios where the opponent lies about their intentions. In general, this section shows how language can be used to form beliefs over hidden mental states.



% \subsection{Beliefs over Values}
% \textbf{Problem Formulation.} How can we form a belief over the preferences of an agent based on its actions? To test this, we consider a game of barter where an agent must trade 

% \textbf{In-Context Demonstrations.} We demonstrate (or teach) the model how to search and evaluate in the continuous action space with two demonstrations with trivial payoff functions.

% \textbf{Evaluation Tasks.} The evaluation is performed with unseen payoff functions. We test two classes of polynomial equations (binomial and trinomial) with five sets of coefficients each.

% \textbf{Results.} 


\vspace{-0.1cm}
\subsubsection{Realistic Scenario: Model as a negotiator}

In this section, we test if a model can negotiate with a human in a complex realistic negotiation setting by forming a belief over their values through multiple rounds of interaction. 

\textbf{Experiment Setup.}We use the Deal or No Deal environment \citep{lewis2017deal} to test our method (\autoref{fig:dealnodeal}). We restrict negotiations to a three turn (6 offers) setting. The human gets a chance to first propose an offer and then agents can propose a counter offer or accept/ reject the offer. When an agent rejects an offer, the player get no reward. Demonstrations (\autoref{fig:dealnodeal}b) are provided by an expert human player collected while playing against another human. These are then annotated systematically by the player to generate 7 demonstrations. The demonstrations capture the style of the human player.

We evaluate the model on new negotiating partners in settings with new values and item quantities. We consider two baselines to compare our models against: 1) A few shot baseline without chain of thought prompting, 2) prompting with strategic reasoning without explicitly forming beliefs over the values of the other player. We conducted a user study with 11 human participants that were asked to interact with the three negotiation methods for three episodes each. After interacting with the agents, the participants are asked to fill out a survey, rating the agent on different aspects of their negotiating ability on a 7-point Likert scale. Participants rated how human-like, reasonable, aggressive or compromising an agent was.


\textbf{Results.} Our method outperforms baselines on multiple metrics (\autoref{fig:deal-res}), achieving a higher average reward (7.6) compared to the `no belief' model (6.7) and the few-shot baseline (4.8). Despite our model getting a higher reward, the humans received a similar (slightly higher) reward when negotiating with our method. We are successfully able to build a negotiating agent with no additional training, only through few-shot demonstrations. Further, the agent mimics the style of the human which is reflected in the post-study survey; as our agent was consistently rated to be more human-like, reasonable, compromising and less aggressive. 





% \begin{itemize}
%     \item Challenges: Modelling opponents values, Coming up with good proposals for yourself and opponent based on beliefs of what the opponent likes
%     \item Prompting: Modelling beliefs, evaluating proposals, coming up with counter proposals
%     \item Human user study w/ GPT, CODEX negotiator (or only CODEX)
%     \item Baseline: Human deal negotiated in the dataset
%     \item Optional: Different characteristics of the negotiator based on demonstrations
%     \item Optional: Soft definition of objectives for the negotiator. Eg: Want more value than 5, Get me the book no matter what the value is given
%     \item How sensible the model was
%     \item External labeler how good a negotiation was or which one is better based on ranking
%     \item N=3x3x10 w/ H=10+
% \end{itemize}
